Kvasir-SEG: A Segmented Polyp Dataset

Pixel-wise image segmentation is a highly demanding task in medical-image analysis. In practice, it is difficult to find annotated medical images with corresponding segmentation masks. In this paper, we present Kvasir-SEG: an open-access dataset of gastrointestinal polyp images and corresponding segmentation masks, manually annotated by a medical doctor and then verified by an experienced gastroenterologist. Moreover, we also generated the bounding boxes of the polyp regions with the help of segmentation masks. We demonstrate the use of our dataset with a traditional segmentation approach and a modern deep-learning based Convolutional Neural Network (CNN) approach. The dataset will be of value for researchers to reproduce results and compare methods. By adding segmentation masks to the Kvasir dataset, which only provide frame-wise annotations, we enable multimedia and computer vision researchers to contribute in the field of polyp segmentation and automatic analysis of colonoscopy images.

==> reviewers_comments.tex <==


##################Reviewers comments#########################################
# Reviewer 1


The paper introduces a new image segmentation dataset (1000 images) comprised of gastrointestinal polyp images with their corresponding segmentation masks. The dataset is an extension of another image classification dataset consisting of 8000 images and eight classes. The intended segmentation task for the introduced dataset is evaluated using two baseline approaches: Fuzzy C-mean clustering (FCM) as well as a Deep Residual U-Net (ResUNet). Evaluations using Intersection over Union and Dice coefficient show that the ResUNet outperforms FCM by a large margin.

The text is written well and the dataset's purpose is explained in great detail. However, the text also includes some redundancies, while in other parts lacks clarity (see suggestions). Nevertheless, the dataset is a fine contribution to the medical multimedia community, especially considering the sparse availability of such datasets.

Suggestions
--------------

Content:

- ... Kvasir-SEG: an open-access dataset of gastrointestinal polyp images and corresponding segmentation masks, manually annotated and verified by an experienced gastroenterologist. -> One person should not do both, annotating and evaluating -- as is as well stated in the text, this makes annotations subject to physician’s bias or inter-observer variation. It is clear that this is hard to rectify for this dataset, but should be considered for future extensions.HDJ: Not much we can do here. Reviewer says it should be considered for the future.

PH: Well the procedure was that D and Pia annotated and THEN Tomas verified. Maybe just add "...THEN verified..."


- We manually annotated and labeled all of the 1000 images with the help of [medical experts -> a medical expert]. -> It is assumed the experienced gastroenterologist is addressed here?


Fixed please check. 



- In this respect, we [have released -> release] the Kvasir-SEG dataset and [proposed -> propose] a baseline model ... -> Since this dataset is introduced with the paper, it should be referred to in present tense.

Fixed

- Kvasir 1.0 vs Kvasir 2.0 vs Kvasir-Seg: It is not really clear why Kvasir-Seg is brought in relation to Kvasir 1.0/2.0. As is understood from the text Kvasir-Seg does not contain any images from Kvasir nor is it made for eight different polyp classes. It, therefore, rather seems like an entirely new dataset rather than an "extension". In fact, a reader could very likely be confusing the extension of Kvasir 1.0, i.e. Kvasir 2.0, with Kvasir-Seg as it is called an "extension" in the Introduction -- the provided dataset link (that should btw. not be added to an anonymous paper) clarified this for me, but it would be beneficial for the paper to be more precise on this.

We have to discuss.

PH: I Would dropp the v1 vs v2. Describe Kvasir v2 as Kvasir and remove the v1 stuff.



- ... open-access dataset for consistent evaluation is missing in this field. -> What exactly is "consistent evaluation"? Why can novel approaches not be evaluated on the other referenced datasets? (Researchers are perfectly capable of online registration/contacting dataset owners) This should be clarified/motivated better, or omitted.

We have to discuss. 


- The open-access dataset can be easily downloaded for research purposes at: [https://datasets.simula.no/kvasir/ -> https://datasets.simula.no/kvasir-seg/).

Fixed.


- This dataset can assist the development of state-of-the-art solutions on images captured by colonoscopes from different manufacturers. -> Why "different manufacturers"? Have there been several different colonoscopes used during the collection of the dataset? If so, this should be stated.

We have to fix together. 


- ... we resized our dataset to into 320 × 320 pixels. -> What is the original image resolution?

Fixed. (have to mention in the paper)

- For fairness, we have included the training, validation and testing scores ... -> What exactly is addressed with the word "fairness"?

We have to discuss.

- Redundancies: The following text passages feel redundant to read, consider removing repetitions/shortening them: 5, 5.1, 5.3

We have to discuss.

- Fig. 4: The image looks squeezed -- consider resizing it preserving its original width/height ratio.

We have to solve this. 

Textual:
- generally: often articles are omitted, which should be corrected, e.g.: [More -> A more] detailed explanation ... can be found; ... dataset was used for [multimedia -> the multimedia] challenge ...; predict the ground truth on [Kvasir -> the Kvasir] dataset; because of [unavailability -> the unavailability] of ground truth information ...

- ... it is difficult to find annotated medical images with corresponding segmentation [mask -> masks].

Fixed. 

- [Polyps are -> A polyp is an] abnormal tissue growth from the mucous ...

Fixed

- In addition, several studies [has -> have] shown that polyps ...
Fixed

- The [Region -> Regions] of Interest (ROI) are the pixels ...

Fixed

- For the experiment, we have used [Fuzzy C-mean clustering algorithm [6] -> Fuzzy C-mean clustering algorithm (FCM) [6] ] ...
Fixed

- We conclude our work and give future [direction -> directions] in Section 6.

Fixed

- Riegler et al. [18] have raised several open questions about the medical world that [needs -> need] to be addressed ...
Fixed


- ... we noticed that the model [were -> was] getting overfitted ...
Fixed

- ... model can be improved by [presenting it -> providing it with] more unique polyp images.

Fixed

- Our results show that the ResUNet model [was -> is] superior to FCM clustering.
Fixed

# # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # ###Reveiewer's comments###################################
# Reviewer 2

This work presents an extension of the KVASIR dataset (which contains images of different classes belonging to different medical findings in the human GI tract) with segmentation masks of the 'polyp' class - which is probably one of the most important classes, since polyps are precursors for colorectal cancer. The segmentation masks have been verified by a gastrointestinal expert. The dataset can be used to design and evaluate region segmentation methods for the purpose of polyp segmentation. The authors also suggest the well-known Dice and Intersection-over-Union (IoU) metrics to be used when performing evaluations with this dataset and provide an initial evaluation with FCM clustering and the ResUNet network, which achieves a quite promising segmentation performance of a mean Intersection-over-Union of 70.15%.

The paper is a perfect fit for the MDRE special session and is expected to have high impact to the multimedia community too, which is increasingly focusing on the medical multimedia domain as well.

It is a pity though that the dataset does not contain bounding boxes as well (although they could be automatically computed for the segmentation masks), since segmentation methods are often evaluated on both pixel-wise segmentation and bounding-box-based localization.

We have to discuss. (and fix)

Please correct these typos:
"with age [20]" -> "with age [20]." (minor typo, but still there should be a point in the end of the sentence)

FIxed
"the pixels covered by the outline in the Figure 1 shows" -> "the pixels covered by the outline in Figure 1 show"

Fixed

"In addition, several studies has shown" -> "In addition, several studies have shown"
Fixed

###########################################################################################################################################################################


Reviewer's comments::
Review 3


This paper presents an extended version of the Kvasir dataset, which the polyp images associate with their segmentation masks. The paper also proposes a set of metrics, that helps researchers to have a better and standard ways for comparing and evaluating. The paper is well written and easy to follow, the SoA is up to date. I would recommend this study for publication.






# # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # # #

# Reviewer's comment

Review 4

In this work, the authors propose Kvasir-SEG, an open access dataset of gastrointestinal polyp images and corresponding segmentation masks that were manually generated by an expert. The dataset is an extension of the Kvasir dataset by the inclusion of the segmentation masks for a subset of the images (1000?).

The motivation for the dataset is good and there are extensive references provided.

The inclusion of metrics and strong baselines were also a good addition that strengthens the paper.

==> takeouts.tex <==
Medical image segmentation can assist processes such as monitoring pathology, improving the diagnostic ability, and facilitate physicians and radiologists in diagnosing diseases such as cancer, inflammation and injury. For the medical images, it is important to understand at pixel label than at image label. The large volume of medical (3D and 4D) images are being stored and processed, and their information is being utilized for the experiment. Therefore, there is a need for an automated and efficient image segmentation technique. To enable automated \ac{CAI}, pixel-wise semantic segmentation methods have a huge potential to become part of a fast, accurate and cost-effective system. A CAI system can facilitate the clinical pathway of a significant number of patients more efficiently than ever before. However, for the system to be used in clinical settings, it should be able to make accurate prediction on challenging images as well (for example, presence of blood or motion artifacts). All these factors should be considered in the early stages of developing automatic and efficient CAI systems.  



\section{Applications}
\label{sec:Application}
The Kvasir-SEG dataset is intended to be used for researching and developing new and improved methods for detection, localization, and classification of polyps.
Multiple datasets are prerequisites for comparing computer vision based algorithms, and this dataset is useful both as a training dataset or as a validation dataset. This dataset can assist the development of state-of-the-art solutions on images captured by instruments from different manufacturers. Further research in this field has the potential to help reduce the polyp-miss rate and thus improve examination quality.

The Kvasir-SEG dataset is also suitable for general segmentation research. In this context, the dataset can accompany several other datasets from a wide range of fields, both medical and otherwise. 

The Kvasir-SEG is also essential because it is challenging to collect a large volume of annotated GI tract images, let alone images of polyps. Among the collected video frames, some  are corrupted heavily with multiple artifacts. Most datasets released on polyps does not contain annotated segmentation masks, but it is rather bounding boxes or whole images which are annotated as containing polyps. One advantage of pixel wise segmentation of polyps may be a more precise ground truth for the neural networks to learn from. Hopefully, this can contribute to more exact predictions and better results. In a colonoscopy setting, polyps might present as small lesions covering a limited number of pixels in each frame, sometimes only visible in a few frames only. This is important to take into account when developing algorithms with the purpose of detecting polyps. 

Moreover, the literature review also shows that there are only limited available datasets. Among them, the use for some of them are restricted, and one needs to obtain permission to use them. Also, the datasets are captured using the same colonoscopic equipment and the size of the datasets are minimal. 




For the medical images, it is important to understand at pixel label than at image label. 

The large volume of medical (3D and 4D) images are being stored and processed, and their information is being utilized for the experiment. 

A CAI system can facilitate the clinical pathway of a significant number of patients more efficiently than ever before. 

However, for the system to be used in clinical settings, it should be able to make accurate prediction on challenging images as well (for example, presence of blood or motion artifacts). 

All these factors should be considered in the early stages of developing automatic and efficient \ac{CAI} systems.  

Something about how image segmentation is a key part of automatic detection.Image segmentation is the technique of dividing images into meaningful regions that are simple to analyze and interpret.It also needs to accept and process images or videos captured at different hospitals  using devices from a variety of manufacturers.


Moreover, multimedia researchers can use the dataset as common dataset for the experiment and develop 
new models or . 
the multimedia researchers should collect and annotate more datasets like ours for developing more efficient models.
more datasets like ours would be beneficial for developing more efficient models.
containing = depicting 

The Kvasir-SEG dataset can be used as test dataset for the already developed machine learning algorithms . The dataset can also be used to evaluate segmentation algorithms, to compare results with the state-of-the-art algorithms, and contribute to building complete pipelines providing human-level competence in the diagnosis of colorectal cancer. 
In the colonoscopies procedure, to provide a real-time feedback,the image segmentation would be crucial. (may be in application)?

% However, large amount of data is required to make an efficient ML/DL model. Moreover, the dataset outlined above is from the same research group and the dataset are captured using same instrument. The ML/DL models needs test dataset that are completely unseen to avoid biases on a specific dataset. Thus, the Kvasir-SEG dataset has potential of being used as the test dataset for the experiment. The dataset can also be used to evaluate segmentation algorithms, to compare results with the state-of-the-art algorithms, and contribute to building complete pipelines providing human-level competence in the diagnosis of colorectal cancer. In the colonoscopies procedure, to provide a real-time feedback,the image segmentation would be crucial. To meet these needs, it was a necessity to annotate the Kvasir dataset with segmentation masks and making it open access to the multimedia community. Thus, the presented work can be a strong base for addressing the problem of public datasets for evaluation, and be helpful in developing robust and efficient systems.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Basic model 

% Clustering is the process of partitioning the dataset into a similar group such that the dataset belonging to the same group has similar characteristics. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Conclusion


%The Kvasir-SEG dataset can be used for evaluating segmentation algorithms as well as comparing results. %In future, we aim to segment all classes of the  Kvasir~\cite{kvasir} and Nerthus datasets~\cite{Pogorelov:2017:NBP:3083187.3083216}. 

%We hope our efforts will inspire the community to create even larger \ac{GI} datasets.

%This might be beneficial to the endoscopist community, including image analysis, clinical endoscopists, and manufacturers. 
%can be useful towards improving the future health care systems. 
%We also plan to improve the overall performance as well as processing speed by testing with the new available models in order to achieve segmentation goals.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%Discussion%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Few advantages for this algorithm are that no training is required, and efficient on-line execution is possible without GPU.

Color filtering was used to initially generate a mask of
instruments to distinguish from the background, where color
features are extracted using thresholds on the opponent color
space and hue/saturation channels.

https://arxiv.org/pdf/1902.06426.pdf


